DeLTA: GPU Performance Model for Deep Learning Applications with In-depth Memory System Traffic Analysis

Training convolutional neural networks (CNNs) requires intense compute throughput and high memory bandwidth. Especially, convolution layers account for the majority of the execution time of CNN training, and GPUs are commonly used to accelerate these layer workloads. GPU design optimization for efficient CNN training acceleration requires the accurate modeling of how their performance improves when computing and memory resources are increased. We present DeLTA, the first analytical model that accurately estimates the traffic at each GPU memory hierarchy level, while accounting for the complex reuse patterns of a parallel convolution algorithm. We demonstrate that our model is both accurate and robust for different CNNs and GPU architectures. We then show how this model can be used to carefully balance the scaling of different GPU resources for efficient CNN performance improvement.

==> Makefile <==
all:  main.tex bib/*.bib IEEEtran.cls
	pdflatex main
	bibtex main
	pdflatex main
	pdflatex -synctex=-1 main
	sed -i -e 's/build_tex/tex/g' -e 's/\/cygdrive\/c/C:/g' main.synctex
	#gs -sOutputFile=main_bw.pdf -sDEVICE=pdfwrite -sColorConversionStrategy=Gray -dProcessColorModel=/DeviceGray -dCompatibilityLevel=1.4 -dNOPAUSE -dBATCH main.pdf
clean: 
	rm -rf *.aux *.bbl *.blg *.log *.out main.pdf main_bw.pdf main.dvi main.synctex


==> tex/generalization.tex <==
\section{Conclusion}
\label{sec:general}

[Maybe this should be part of conclusion?]
Although we model the memory traffic with im2col algorithm based matrix convolution workloads on Pascal GPU architecture, the proposed mechanism can be generalized to other GPU designs and convolution algorithms. We can predict the data load traffic at L1 channel by calculating the effective range of data elements touched by each warp which we defined as EEPW. The size of EEPW can vary depending on the kernel design but the mechanism remains the same. We estimated L2 traffic using intra-CTA data reuse and this mechanism can be applied to other algorithms such as FFT and Winograd. These algorithms have less data reuse within each matrix multiplication block can reuse the data reduce the reuse thus increase the data load traffic per request. On the other hand, bigger convolution GEMM blocking factor increase reuse thus reduce L2 traffic. Finally, understanding how CTAs are scheduled and how data elements are reused among CTAs can be used to predict the data traffic at DRAM channels. The size of L2 cache compared to the footprint of the entire workload or blocked working set impacts the prediction accuracy.

==> tex/l2_temp.tex <==
\subsection{L2 Cache Traffic}
\label{sub_sec:l2_model}

% === Should have an overview statement
%L1 cache is dedicated to a single SM and each SM executes one or more CTAs.
%We assume that L1 can capture the temporal and spatial data locality of the same CTA, but not the inter-CTA reuse due to its relatively small size.
%With this assumption, our L2 traffic model estimates the traffic by identifying the unique data accesses per CTA.

In im2col GEMM, the IFmap matrix with many duplicated data accesses involves high spatial and temporal locality.
As L1 cache is dedicated to a single SM, L1 can capture the reuse within one CTA's IFmap tile but not across active CTAs per SM given its small size ($\sim$32KB).
With this assumption, our L2 model estimates the traffic by identifying the unique data accesses made in CTA input tile.

%Due to repeated use of the same data, the same cacheline is accessed multiple times. 
%We assume that the L1 cache can deliver data for the repeated accesses from the same CTA, but cannot capture inter-CTA reuse due to its relatively small size.
%With this assumption, our model uses each CTA's blocked GEMM input tile as memory access block to L2 and 
%calculates the traffic using the average unique data elements in each blocked GEMM input tile and the number of input tiles per CTA.

%===== CTA tile configuration and its impact
\textit{\textbf{CTA Tile Selection.}}
%We first set the CTA tile size for a given Conv layer as it affects the number of reusable data elements within CTA's main loop iteration
CTA tile size affects the spatial locality of the data elements accessed by a CTA; a bigger CTA tile has more data reuse.
%Also, the CTA tile size determines the number of CTAs per workload and the ratio between math operations and memory loads per main loop iteration. 
%Therefore, CTA tile size is carefully chosen as it affects the number of CTAs per workload and the ratio between math operations and memory loads per loop iteration~\cite{lai2013performance}. 
It also affects the number of CTAs per workload and the ratio between math operations and memory loads per main loop iteration. 
As it is a critical factor in modeling memory traffic, we analyze the CTA tile size (\((blk_M + blk_N) \times blk_K\)) of the potential convolution GEMM kernels. 
Based on our analysis, cuDNN uses three types of CTA tilings: \((128 \times 128)\times 8\), \((128 \times 64)\times 4\), and \((128 \times 32)\times 4\).
\(blk_M\) is fixed to 128 for all tiles and \(blk_N\) is chosen based on the width of the convolution GEMM \((C_o)\). 
We measure the CTA tile size by different \(C_o\) and use this as a look-up table to our L2 traffic model.
%\fig{fig:ifmap_input_tile} shows the CTA tiles used by different different K and we apply this graph as a look-up table to our L2 traffic model.

%===== Coalescing within a ifmap input tile
% ifmap data rearranged => can find many data reuse within a input tile => stride, filter size, feature size
% size of unique data simply equated using two points distance

%%%% CTA tile size scan
%\begin{figure}[t]
%    \centering
%    \includegraphics[width=0.48\textwidth]{fig/cta_tile_size.pdf}
%    \caption{Selected CTA tiles for the convolution layers with different number of OFmap channels \(K\)}
%    \label{fig:ifmap_input_tile}
%    \vspace*{-3mm}
%\end{figure}
%%%% Unique data per IFmap input block
\begin{figure}[t]
    \centering
    \includegraphics[width=0.445\textwidth]{fig/l2.pdf}
    %\caption{\small{IFmap data layout of im2col GEMM. The data in each tile (\(blk_M \!\times\! blk_K \)) are the input for one main loop. The unique data elements are represented by \(DIST_V\) and \(DIST_H\). The data in the white dotted boxes show the spatial reuse pattern within an IFmap tile.}}
    \caption{\small{IFmap data layout of im2col GEMM. The elements in \(blk_M \!\times\! blk_K \) IFmap tile are the input for one main loop. Other details on the figure are described in \sect{sub_sec:l2_model}.}}
    \label{fig:l2_dist}
    \vspace*{-4mm}
\end{figure}
%\textit{\textbf{IFmap data traffic.}} 
\textit{\textbf{Intra-CTA Spatial Locality.}}
We extend the example used in \sect{sub_sec:l1_model} to explain our L2 traffic model (\fig{fig:l2_dist}).
Again, IFmap elements visited by one filter data are remapped as a column in the IFmap matrix (\textcolor{red}{\ding{182}}) and the next column contains the IFmap data traversed by another filter data (\textcolor{blue}{\ding{183}}). 
Therefore, a \(blk_M \!\times\! blk_K\) IFmap tile for one main loop iteration consists of multiple copies of data that are in continuous address range.
This access pattern entails large data locality shown by the duplicated data element in the white doted boxes.
As L1 cache captures the locality within each tile, only the unique elements are requested to L2.
Thus, based on our observation, if we know the address range of data within one IFmap tile (difference between the smallest and the largest address), we can estimate the size of memory requests to L2 in the tile.
To be specific, within each IFmap tile, the accessed address increases from the top to the bottom and left to the right.
Therefore, the sum of the address distances between A and B (both edges of \(blk_M\)), and B and C (both edges of \(blk_K\)) in \fig{fig:l2_dist} estimates the total accessed data within an IFmap tile.

%Different filter data elements visit many overlapping IFmap data.
%This spatial reuse pattern is shown by the elements in the white doted boxes and this changes depending on the filter size, stride, and IFmap size.
%The data elements within a \(blk_M \!\times\! blk_K\) tile are used as inputs in a main loop iteration and the locality within this tile can be captured by L1. 
%Therefore, only the unique elements within a tile are delivered from L2.

%We found that the sum of the vertical and horizontal data ranges of one IFmap tile (red colored boxes) effectively represents the unique data elements accessed. 
%We found that the distances of vertical and horizontal data elements of one IFmap tile (elements in the black dotted boxes) effectively represents the unique data elements accessed within an IFmap tile.
We first define the address distance between A and B as {\small\(DIST_V\)} (vertical distance).
As the data elements in a column are the IFmap data traversed by one filter data, we formulate {\small\((DIST_V)\)} as \eq{eq:dist_v} using the mechanism used in L1 traffic modeling.
Also, when IFmap tile spans over more than one channel, multiple unique {\small\(DIST_V\)} can be located within an IFmap tile.
In this example, the red and green colored elements belong to different channels.
If an IFmap tile spans these two channels, it needs to fetch the data elements of both channels.
Therefore, the ratio between the channel width and IFmap width affects the average size of vertical distances {\small\((A\_DIST_V)\)}.
We calculate {\small\((A\_DIST_V)\)} using \eq{eq:eff_dist_v} where \(H_f \!\times\! W_f\) indicates the width of a channel.
\eq{eq:eff_dist_v}.
%We calculate the average vertical distance per IFmap tile  as \eq{eq:eff_dist_v}.
%\begin{equation}
%\scriptsize
%\label{eq:dist}
%DIST_{GEMM\_tile} = DIST_{V} + DIST_{H}
%\vspace*{-2mm}
%\end{equation}
\begin{equation}
\scriptsize
\label{eq:dist_v}
%DIST_{V} = \frac{DISTance\ of\ elements}{blk_M} = blk_{M} \times \frac{(H_i+2Pad) \times Strd}{H_i+2Pad-S+1}
DIST_{V} = blk_{M} \times \frac{(W_i+2Pad) \times Strd}{W_i+2Pad-Wf+1}
\end{equation}
\begin{equation}
\scriptsize
\label{eq:eff_dist_v}
%    E\_DIST_{V} = 
%\begin{cases}
%    DIST_V \times \frac{blk_K}{S}&, \text{if } Strd = 1\\
%    DIST_V \times \frac{blk_K}{R \times S}&, \text{otherwise}
%\end{cases}
A\_DIST_{V} = DIST_V \times \frac{blk_K}{H_f \times W_f}
\end{equation}

% Horizontal distance
Next, we define the address distance between B and C of an IFmap tile as {\small\((DIST_H)\)} (horizontal distance).
Based on our observation, the distance between two adjacent columns within the same \(W_f\) range is 1 (\ding{184}) as they are traversed by the two adjacent element of a filter.
However, the distance between two columns in different \(W_f\) ranges is {\small\(W_i\!+2Pad-W_f+1\)} (\ding{185}) which is determined by the size of an IFmap.
%is set by the filter element traversal on an IFmap.
%However, the distance between the two columns in different \(W_f\) ranges is {\small\(W_i\!+2Pad-W_f+1\)} (\ding{185}) which is set by the filter data location in the next row of IFmap.
Also, the alignment of the filter width (\(W_f\)) to \(blk_K\) affects the number of \(H_f\) edges within an IFmap tile.
Therefore, considering both the inter-column distances and the alignment to \(blk_K\), we calculate {\small\(DIST_H\)} using \eq{eq:dist_h}.
%Using these inter-column distances within an IFmap tile and considering the alignment of the filter width (\(S\)) to the blocking factor (\(blk_K\)), {\small\(DIST_H\)} can be calculated using \eq{eq:dist_h}.
%Also, the size of the convolution stride affects the expected {\small\(DIST_H\)}. 
%When \(filter\ stride > 1\), the data elements in horizontal direction at every {\small\((H+2Pad-R+1)\)} are unique and it is {\small\((H+2Pad-R+1)^2\)} for the stride is 1.
%\eq{eq:eff_dist_h} reflects such variation and calculates the expected horizontal distance {\small\((E\_DIST_H)\)}.
Like the vertical distances, if one IFmap spans more than one data sample, multiple unique {\small\({DIST_H}\)} can be found within an IFmap tile.
For example, in \fig{fig:l2_dist}, the light colored red and green elements belong to a different sample.
Therefore, the number of unique horizontal distances per IFmap is affected by the ratio between the IFmap height (\(blk_M\)) and the entire elements traversed by one filter element \((\frac{W_i+2Pad-W_f+1}{Strd})^2\) (assuming height and width are the same).

%If the elements of more than one data sample are located within a IFmap tile, multiple unique {\small\({DIST_H}\)} can be found within an IFmap tile.
In \fig{fig:l2_dist}, the data elements of two different samples present within a \(blk_M\) range which adds an additional {\small\(DIST_H\)} (horizontal blue dotted box).
The number of samples per IFmap tile is affected by the ratio between \(blk_M\) and the size of one IFmap which is the product of the height and width of an IFmap or \((\frac{W_i+2Pad-W_f+1}{Strd})^2\) (assuming height and width are the same).
%Thus, the average number of the unique \(DIST_H\) within a input tile depends on the ratio between the height of a input tile \((blk_M)\) and the size of one IFmap converted to a GEMM input column \((\frac{W_i+2Pad-W_f+1}{Strd})^2\).
%Also, if the size of a feature is smaller than the CTA height blocking factor (\(blk_M\)), more than one \(DIST_H\) can exist within a input tile (elements in the horizontal blue dotted box).
%Thus, the average number of the unique \(DIST_H\) within a input tile depends on the ratio between the height of a input tile \((blk_M)\) and the size of one IFmap converted to a GEMM input column \((\frac{W_i+2Pad-W_f+1}{Strd})^2\).
Reflecting this, we calculate the average horizontal distance of an IFmap tile {\small\((A\_DIST_H)\)} (\eq{eq:eff_dist_h}).
\begin{equation}
\scriptsize
\label{eq:dist_h}
\begin{split}
    DIST_H  &= \Big( \frac{blk_{K} \!-1}{W_f} \Big) \!\times\! \big( (W_i \!-\! W_f+1) + Strd \!\times\! (W_f \!-\! blk_{K} \!+\! 1) \big)\\
            &+ \Big( \frac{W_f-blk_K+1}{W_f} \Big) \times \big( Strd \!\times\! (blk_K-1) \big)
\end{split}
\vspace*{-3mm}
\end{equation}
\begin{equation}
\scriptsize
\label{eq:eff_dist_h}
%    E\_DIST_{H}= 
%\begin{cases}
%    DIST_H \!\times\! \big( 1+ \ceil{\frac{blk_M}{(H+2Pad-R+1)^2}} \big) \!\!\!&, \text{if } Strd = 1\\
%    DIST_H \!\times\! \big( 1+ \ceil{\frac{blk_M}{H+2Pad-R+1}} \big)&,               \text{otherwise}
%\end{cases}
%E\_DIST_{H} = DIST_H \!\times\! \Big( 1+ \ceil{\frac{blk_M}{(\frac{H+2Pad-R+1}{Strd})^2}} \Big)
A\_DIST_{H} = DIST_H \!\times\! \Big( 1+ \frac{blk_M}{\big(\frac{H_i+2Pad-H_f+1}{Strd}\big)^2} \Big)
\end{equation}

%===== 1x1 convolution and total L2 traffic euqation
In case of \(1 \!\times\! 1\) convolution and FC layers, all IFmap data elements are unique and there is no data reuse within an IFmap tile.
Therefore, we can simply calculate {\small\(DIST_V\)} as the height of an IFmap tile and {\small\(DIST_H\)} as its width.
The same method is applied to filter data elements because they are all unique as well.
Finally, using the expected distance of IFmap and filter tiles, the total L2 load traffic within a main loop is calculated by adding {\small\(A\_DIST_V\)} and {\small\(A\_DIST_H\)}.
Then, the total L2 traffic for a Conv layer is calculated by considering the number of CTAs and the number of main loop iterations (\eq{eq:l2_traffic}).
\begin{equation}
\scriptsize
\label{eq:l2_traffic}
\begin{split}
T_{L2\_total}   &= A\_DIST_{GEMM\_tile} \times \frac{GEMM\ tiles}{Conv\ layer}\\
                &= \big(A\_DIST_{IFmap} + DIST_{Filter} \big) \!\times\! \frac{K}{blk_K} \!\times\! \frac{N_{CTA}}{Conv\ layer}
\end{split}
\end{equation}

% =================== Cached
%The horizontal distance is set by the number filter data (each becomes one column in IFmap tile) traversing one IFmap matrix. For example, \(ith\) IFmap tile indicated by \(blk\_K_{(i)}\) has the IFmap data elements traversed by 3 rows and (3, 3, 2) columns in each row of the filter matrix. The distance between two rows in a filter matrix is \(W-R+1\) and the distance between columns within the same row equals to the filter stride. Using this relation between the data points in IFmap tile, we can calculate the expected horizontal distance. The horizontal distance is set differently depending on the size of filter and the width of input tile \((bkl_K)\). When \(blk_K\) is bigger than or equal to the filter height (and width), an IFmap tile always includes the data elements traversed by \(\floor{\frac{blk_{K}}{S}}\) columns in the filter matrix. However, if the input tile width is smaller than the filter height (and width), depending on the alignment between the IFmap tile and the IFmap columns, IFmap tile can only contain the data elements visited by the data elements in the same filter matrix row. \eq{eq:dist_h} and \eq{eq:dist_h} reflects the average difference between two cases.

%Unlike the IFmap tile, data elements in one filter tile are all unique meaning no request coalescing and reuse at L1 cache. Also, as the global loads are served in sectors, the data larger than input tile is loaded. However, L1 cache support the short data reuse distance of a single loop iteration so we simply calculate the L2 load transactions for filter data as \(blk_N \times blk_K\). Then, the total L2 transactions for one main loop is calculated by adding \(DIST_V\), \(DIST_H\), and \(blk_N \times blk_K\) and the total L2 traffic per layer workload is calculated as: 

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> tex/overview.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{overview}

\noindent\textbf{\emph{Motivation.}}
\begin{itemize}[noitemsep,topsep=5pt,leftmargin=0.15in]
    \item Deep learning kernels are designed to maximize GPU computing unit utilization as they are computation intensive in general
    \item As GPU's compute throughput increases with larger number of cores or more SIMD units per core (or tensor cores), deep learning workload execution time is expected to be also restricted by the memory system
    \item Existing GPU performance models assume the deep learning kernels are bottlenecked by compute throughput thus do not model memory system in detail
    \item It is important to improve GPU HW resource efficiently so it leads to the optimal deep learning application performance with minimum needed cost
\end{itemize}

\noindent\textbf{\emph{Contribution.}}
\begin{itemize}[noitemsep,topsep=5pt,leftmargin=0.15in]
    \item We analyze and model the memory traffic and the cache hit rate of deep learning applications running on GPU
    \item We analyze deep learning application performance where the kernel execution is bottlenecked not only by computation throughput but by the memory system bandwidth using our model
    \item We analyze the performance trade-offs in kernel configuration and HW resource cost
    \item We discuss and suggest the optimal options of deep learning application kernel configuration and resource requirement for the performance of deep learning applications
\end{itemize}

\noindent\textbf{\emph{Background.}}
\begin{itemize}[noitemsep,topsep=5pt,leftmargin=0.15in]
    \item Convolution lowering for deep learning application execution parallelism for GPU
    \item GPU CTA tiling mechanism and resource allocation
    \item Convolution kernel design and work process
    \item Prior work on GEMM performance modeling
\end{itemize}

\noindent\textbf{\emph{Main Idea.}}
\begin{itemize}[noitemsep,topsep=5pt,leftmargin=0.15in]
    \item Data locality in convolution matrix
    \item L1 traffic: Sector based memory queries, Memory access inefficiency associated with kernel stride
    \item L2 traffic: Input tensor size and its ratio to cache capacity
    \item DRAM traffic: Data locality within CTA and inter-CTA (sliding window)
    \item Multi-warp / Multi-CTA scheduling and its impact to GPU execution time
\end{itemize}

\noindent\textbf{\emph{Experiment.}}
\begin{itemize}[noitemsep,topsep=5pt,leftmargin=0.15in]
    \item GPU performance estimation with compute throughput scaling
    \item GPU performance bottleneck points with varying GPU HW resource configurations
    \item GPU performance bottleneck points with varying kernel designs
\end{itemize}

